The Bit Complexity of Dynamic Algebraic Formulas and their Determinants

Many iterative algorithms in optimization, computational geometry, computer algebra, and other areas of computer science require repeated computation of some algebraic expression whose input changes slightly from one iteration to the next. Although efficient data structures have been proposed for maintaining the solution of such algebraic expressions under low-rank updates, most of these results are only analyzed under exact arithmetic (real-RAM model and finite fields) which may not accurately reflect the complexity guarantees of real computers. In this paper, we analyze the stability and bit complexity of such data structures for expressions that involve the inversion, multiplication, addition, and subtraction of matrices under the word-RAM model. We show that the bit complexity only increases linearly in the number of matrix operations in the expression. In addition, we consider the bit complexity of maintaining the determinant of a matrix expression. We show that the required bit complexity depends on the logarithm of the condition number of matrices instead of the logarithm of their determinant. We also discuss rank maintenance and its connections to determinant maintenance. Our results have wide applications ranging from computational geometry (e.g., computing the volume of a polytope) to optimization (e.g., solving linear programs using the simplex algorithm).

==> dznotes.tex <==
We want to show that in Theorem 3.1 of the SOSA paper, $\|N\|_F$ and $\|N^{-1}\|_F$ are bounded by $\poly(\kappa)$, where $\kappa$ is an upper bound on the $\|\cdot\|_F$ of input matrices.

\begin{lemma}
    Let
    \begin{align*}
        G(A,B,C,D):=\begin{bmatrix}A&B\\C&D\end{bmatrix}\\
    \end{align*}
    Then,
    \begin{align*}
        \|G(A,B,C,D)\|_F\le \|A^{-1}\|_F+\|(D-CA^{-1}B)^{-1}\|_F(\|A^{-1}\|_F\|B\|_F+1)(\|A^{-1}\|_F\|C\|_F+1)
    \end{align*}
\end{lemma}

\begin{proof}
    \begin{align*}
        G(A,B,C,D)^{-1}&=\begin{bmatrix}
            A^{-1}+A^{-1}B(D-CA^{-1}B)^{-1}CA^{-1}&-A^{-1}B(D-CA^{-1}B)^{-1}\\
            -(D-CA^{-1}B)^{-1}CA^{-1}&(D-CA^{-1}B)^{-1}
        \end{bmatrix}\\
        \|G(A,B,C,D)^{-1}\|_F&\le \|A^{-1}+A^{-1}B(D-CA^{-1}B)^{-1}CA^{-1}\|_F+\|A^{-1}B(D-CA^{-1}B)^{-1}\|_F+\|(D-CA^{-1}B)^{-1}CA^{-1}\|_F+\|(D-CA^{-1}B)^{-1}\|_F\\
        &\le \|A^{-1}\|_F+\|(D-CA^{-1}B)^{-1}\|_F(\|A^{-1}\|_F\|B\|_F+1)(\|A^{-1}\|_F\|C\|_F+1)
    \end{align*}
\end{proof}

\paragraph{One gate}
$M_v$ is the $n_v\times m_v$ input matrix.

\begin{align*}
    N^{-1}=N&=\begin{bmatrix}
        I^{(n_v)}&M_v\\
        0^{(m_v,n_v)}&-I^{(m_v)}
    \end{bmatrix}\\
    \|N^{-1}\|_F=\|N\|_F&\le \sqrt{n_v+m_v}+\|M_v\|_F
\end{align*}

\paragraph{Inversion}

$N'$ is a $n_{N'}\times n_{N'}$ matrix. $(N'^{-1})_{I',J'}$ is the $n_w\times n_w$ matrix that the child node $w$ outputs.
\begin{align*}
    N&=\begin{bmatrix}
        N'&-I^{(n_{N'})}_{[n_{N'}],J'}\\
        I^{(n_{N'})}_{I',[n_{N'}]}&0^{(n_w,n_w)}
    \end{bmatrix}\\
    \|N\|_F&\le \|N'\|_F+\sqrt{n_{N'}+n_w}\\
    \|N^{-1}\|_F&\le \|N'^{-1}\|_F+\|(N'^{-1})_{I',J'})^{-1}\|_F(\|N'^{-1}\|_F\sqrt{n_w}+1)^2
\end{align*}

There is a quadratic dependence on $\|N'^{-1}\|_F$ due to the top left block of $G(A,B,C,0)^{-1}$ being $A^{-1}-A^{-1}B(CA^{-1}B)^{-1}CA^{-1}$.

In our case, we have $A=N',B=-I^{(n_{N'})}_{[n_{N'}],J'},C=I^{(n_{N'})}_{I',[n_{N'}]}$.

Writing $A^{-1}=\begin{bmatrix}
    \alpha&\beta\\
    \gamma&\delta
\end{bmatrix}$ where $(A^{-1})_{I',J'}=\alpha$, we have the top left block of $G(A,B,C,0)^{-1}$ equal to

\begin{align*}
A^{-1}-A^{-1}B(CA^{-1}B)^{-1}CA^{-1}=
    \begin{bmatrix}
        \alpha&\beta\\
        \gamma&\delta
    \end{bmatrix}
    -
    \begin{bmatrix}
        \alpha\\\gamma
    \end{bmatrix}
    \alpha^{-1}
    \begin{bmatrix}
        \alpha&\beta
    \end{bmatrix}=
    \begin{bmatrix}
        \alpha&\beta\\
        \gamma&\delta
    \end{bmatrix}
    -
    \begin{bmatrix}
        \alpha&\beta\\
        \gamma&\gamma\alpha^{-1}\beta
    \end{bmatrix}=
    \begin{bmatrix}
        0&0\\
        0&\delta-\gamma\alpha^{-1}\beta
    \end{bmatrix}
\end{align*}
which is just the Schur complement of $(N'^{-1})_{I',J'}$ of $N'^{-1}$. Does this help at all?

Note that since $\alpha$ and $A^{-1}$ are invertible, $\delta-\gamma\alpha^{-1}\beta$ is invertible and $(\delta-\gamma\alpha^{-1}\beta)^{-1}$ is a block of $A$, namely $(N')_{[n_{N'}]\setminus J',[n_{N'}]\setminus I'}$: by block matrix inversion applied to $A^{-1}$,
\begin{align*}
    (A^{-1})^{-1}=\begin{bmatrix}
        \cdots&\cdots\\
        \cdots&(\delta-\gamma\alpha^{-1}\beta)^{-1}
    \end{bmatrix}
\end{align*}

Formally (permutating the rows and columns), let

\begin{align*}
P_{,I'}&=\begin{bmatrix}
    I^{(n_{N'})}_{I',[n_{N'}]}\\
    I^{(n_{N'})}_{[n_{N'}]\setminus I',[n_{N'}]}\\
    \end{bmatrix}\\
P_{J',}&=\begin{bmatrix}
    I^{(n_{N'})}_{[n_{N'}],J'}&
    I^{(n_{N'})}_{[n_{N'}],[n_{N'}]\setminus J'}
\end{bmatrix}   
\end{align*}
be matrices such that $P_{,I'}X$ permutes rows $I'$ of $X$ to the top, and $XP_{J',}$ permutes columns $J'$ of $X$ to the left.

Since $P^{-1}=P^\top$ for permutation matrices, $P_{,I'}^{-1}=P_{I',}$

Write $P_{,I'}A^{-1}P_{J',}=\begin{bmatrix}
    \alpha&\beta\\\gamma&\delta
\end{bmatrix}$

Then,
\begin{align*}
    \delta-\gamma\alpha^{-1}\beta&=I^{(n_{N'})}_{[n_{N'}]\setminus [|I'|],[n_{N'}]}
    \begin{bmatrix}
    \alpha&\beta\\\gamma&\delta
\end{bmatrix}^{-1}
I^{(n_{N'})}_{[n_{N'}],[n_{N'}]\setminus [|J'|]}\\
&=I^{(n_{N'})}_{[n_{N'}]\setminus [|I'|],[n_{N'}]}
    (P_{,I'}A^{-1}P_{J',})^{-1}
I^{(n_{N'})}_{[n_{N'}],[n_{N'}]\setminus [|J'|]}\\
&=I^{(n_{N'})}_{[n_{N'}]\setminus [|I'|],[n_{N'}]}
    P_{,J'}AP_{I',}
I^{(n_{N'})}_{[n_{N'}],[n_{N'}]\setminus [|J'|]]}\\
&=A_{[n_{N'}]\setminus {J'},[n_{N'}]\setminus I'}&\text{ since $|I'|=|J'|$}
\end{align*}

In particular, $\delta-\gamma\alpha^{-1}\beta=((N')_{[n_{N'}]\setminus J',[n_{N'}]\setminus I'})^{-1}$.

If the child gate was a one (input) gate, this is just $M_v^{-1}$, which is fine.

If the child gate was an add gate, this is (note that $n_w=m_w$ since the output is invertible)
\begin{align*}
    \begin{bmatrix}
        L^{-1}&0&0\\
        0&R^{-1}&0\\
        0&0&0^{(m_w,n_w)}
    \end{bmatrix}
    -
    \begin{bmatrix}
        (L^{-1})_{[n_L],J_L}\\
        (R^{-1})_{[n_R],J_R}\\
        I^{(m_w)}
    \end{bmatrix}
    \begin{bmatrix}
        (L^{-1})_{I_L,J_L}+(R^{-1})_{I_R,J_R}
    \end{bmatrix}^{-1}
    \begin{bmatrix}
        (L^{-1})_{I_L,[n_L]}&
        (R^{-1})_{I_R,[n_R]}&
        I^{(n_w)}
    \end{bmatrix}
\end{align*}

The difficult blocks are the top left block (and symmetrically, the center block). The top left block $L^{-1}-(L^{-1})_{[n_L],J_L}((L^{-1})_{I_L,J_L}+(R^{-1})_{I_R,J_R})^{-1}(L^{-1})_{I_L,[n_L]}$ can also be written as $(L+I_{[n_L],J_L}(R^{-1})_{I_R,J_R}^{-1}I_{I_L,[n_L]})^{-1}$,  since it is the top left block of
\begin{align*}
    \begin{bmatrix}
        L&I_{[n_L],J_L}\\
        I_{I_L,[n_L]}&-(R^{-1})_{I_R,J_R}
    \end{bmatrix}^{-1}
\end{align*}
This doesn't seem helpful though.

If we expand $L^{-1}=\begin{bmatrix}
    a&b\\
    c&d
\end{bmatrix}$ where $(L^{-1})_{I_L,J_L}=a$ and let $z=(R^{-1})_{I_R,J_R}$, then

\begin{align*}
    L^{-1}-(L^{-1})_{[n_L],J_L}(L^{-1})_{I_L,J_L}+(R^{-1})_{I_R,J_R}^{-1}(L^{-1})_{I_L,[n_L]}&=\begin{bmatrix}
        a&b\\
        c&d
    \end{bmatrix}
    -\begin{bmatrix}
        a\\
        c
    \end{bmatrix}
    \begin{bmatrix}
        a+z
    \end{bmatrix}^{-1}
    \begin{bmatrix}
        a&b
    \end{bmatrix}\\
    &=
    \begin{bmatrix}
        a-a(a+z)^{-1}a&b-a(a+z)^{-1}b\\
        c-c(a+z)^{-1}a&d-c(a+z)^{-1}b
    \end{bmatrix}\\
    &=
    \begin{bmatrix}
        a(a+z)^{-1}z&z(a+z)^{-1}b\\
        c(a+z)^{-1}z&d-c(a+z)^{-1}b
    \end{bmatrix}
\end{align*}
The only problematic term seems to be $d-c(a+z)^{-1}b$, as everything else is bounded by $\|L^{-1}\|_F\|R^{-1}\|_F\|\|((L^{-1})_{I_L,J_L}^{-1}+(R^{-1})_{I_R,J_R})^{-1}\|_F$.

Since $z$ is essentially adversarial, we would need a bound on $\sup_{\|x\|_F\le\kappa}\|d-cxb\|_F$. Since we can replace $x$ by $-x$, we need a bound on $\|d\|_F$ (easy) and $\sup_{\|x\|_F\le\kappa}\|cxb\|_F$. I think this is roughly as bad as $\|c\|_F\|x\|_F\|b\|_F$ (take SVD and choose $x$ to align the singular values.), more precisely, $\sigma_{max}(c)^2\sigma_{max}(b)^2\|x\|_F$. So we will probably need a bound on $\|b\|_F\|c\|_F$ for each $L^{-1}$ (i.e. on $\|(N^{-1})_{I',\overline{J'}}\|_F\|(N^{-1})_{\overline{I'},J'}\|_F$) 

For addition gates we already have a duplicated term in this product, but it is also of this form but one level down. Can we bound this inductively?

\paragraph{Addition and Subtraction}

$L$ is a $n_L\times n_L$ matrix and $R$ is a $n_R\times n_R$ matrix.

The outputs of the children gates are $(L^{-1})_{I_L,J_L}$ and $(R^{-1})_{I_R,J_R}$, which are $n_w\times m_w$ matrices.

See SOSA paper for formula of $N$ and $N^{-1}$ (I don't want to typeset it if Jan already has the LaTeX).

\begin{align*}
    \|N\|_F&\le \|L^{-1}\|_F+\|R^{-1}\|_F+\sqrt{2n_L+2n_R+n_w+m_w}\\
    \|N^{-1}\|_F&\le 4\|L^{-1}\|_F+4\|R^{-1}\|_F+\sqrt{n_w+m_w}
\end{align*}

Remark: this gate should generalize straightforwardly to $n$-ary addition.

Remark: we could get a $-(L+R)^{-1}$ gate by taking the bottom-right block of

\begin{align*}
    \begin{bmatrix}
        L&0&I^{(n_L)}_{[n_L],J_L}\\
        0&R&I^{(n_R)}_{[n_R],J_R}\\
        I^{(n_L)}_{I_L,[n_L]}&I^{(n_R)}_{I_R,[n_R]}&0
    \end{bmatrix}^{-1}
\end{align*}

which is shorter.

In fact, the current addition gate (with last two rows swapped) can be viewed as $((L+R)^{-1})^{-1}$ using this, but it somehow avoids problems with $L+R$ not being invertible.

but I think this has the same problems as the inversion gate (e.g. the top left block has a product of two $L^{-1}$ terms.)

\paragraph{Multiplication}
$L$ is a $n_L\times n_L$ matrix, $R$ is a $n_R\times n_R$ matrix.

The outputs of the children gates are $(L^{-1})_{I_L,J_L}$ and $(R^{-1})_{I_R,J_R}$.

\begin{align*}
    N&=\begin{bmatrix}
        L&-I^{(n_L)}_{[n_L],J_L}I^{(n_R)}_{I_R,[n_R]}\\
        0^{(n_R,n_L)}&R
    \end{bmatrix}\\
    \|N\|_F&\le \|L\|_F+\|R\|_F+\sqrt{n_Ln_R}\\
    \|N^{-1}\|_F&\le \|L^{-1}\|_F+\|R^{-1}\|_F(\|L^{-1}\|_F+\sqrt{n_Ln_R})
\end{align*}


\paragraph{For systematic investigation}

Suppose $\|(N^{-1})_{I,J}\|_F$ is bounded by all gates by some universal $\kappa$. (since these are terms that appear in the exact formula).

For each gate, bound $\|N^{-1}\|_F$ and $\|(N^{-1})_{I,[n]}\|_F\|(N^{-1})_{[n],J}\|_F$ in terms of the same kind of terms of its children.

Then, check for which gates can we inductively bound $\|N^{-1}\|_F$ and 
$\|(N^{-1})_{I,[n]}\|_F\|(N^{-1})_{[n],J}\|_F$

I'm thinking of bounding
\begin{align*}
    \|N^{-1}\|_F+\|(N^{-1})_{I,[n]}\|_F\|(N^{-1})_{[n],J}\|_F
\end{align*}

I think addition/subtraction and inverse and multiplication all work out - need to write it up.

TODO: Daniel

\section{2023-06-22}


Write $(N'^{-1})=\begin{bmatrix}
    \alpha&\beta\\
    \gamma&\delta
\end{bmatrix}$ where $\alpha=(N'^{-1})_{I',J'}$

Then,
\begin{align*}
    N'^{-1}-(N'^{-1})_{,J'}(N'^{-1})_{I',J'}^{-1}(N'^{-1})_{I',}&=\begin{bmatrix}
        \alpha&\beta\\
        \gamma&\delta
    \end{bmatrix}
    -
    \begin{bmatrix}
        \alpha\\
        \gamma
    \end{bmatrix}
    \begin{bmatrix}
        \alpha
    \end{bmatrix}^{-1}
    \begin{bmatrix}
        \alpha&\beta
    \end{bmatrix}
    =
    \begin{bmatrix}
        0&0\\
        0&\delta-\gamma\alpha^{-1}\beta
    \end{bmatrix}
\end{align*}

In fact, we have
\begin{align*}
    N^{-1}=\begin{bmatrix}
     0&0&I^{(n_w)}\\
     0&\delta-\gamma\alpha^{-1}\beta&\gamma\alpha^{-1}\\
     -I^{(n_w)}&-\alpha^{-1}\beta&\alpha^{-1}
    \end{bmatrix}
\end{align*}
up to permutation of rows and columns. (TODO: double check)

So,
\begin{align*}
    \|N^{-1}\|_F&\le \sqrt{n_w}+\|N'^{-1}\|_F+\|(N'^{-1})_{I',J'}\|_F(\|(N'^{-1})_{I',}\|_F+1)(\|(N'^{-1})_{,J'}\|_F+1)
\end{align*}
but this bound is worse than not expanding, so seems unecessary.



\section{Recursive norm bounds}
I am using the same notation as the SOSA paper with the additional abbreviation that $A_{I,}=A_{I,[n]}$ and $A_{,J}=A_{[m],J}$ for $A\in\R^{m\times n}$

We want to show that in Theorem 3.1 of the SOSA paper, $\|N\|_F$ and $\|N^{-1}\|_F$ are bounded by $\poly(\kappa)$, where $\kappa$ is an upper bound on the $\|\cdot\|_F$ of input matrices.

We can bound $\|N\|_F$ inductively.

We can bound $\|(N^{-1})_{I,J}\|_F$ using the input constraints.

We can then bound $\|(N^{-1})_{I,}\|_F$ and $\|(N^{-1})_{,J}\|_F$ inductively, and use these to bound $\|N^{-1}\|_F$ inductively. The extra step is to avoid the bound becoming doubly exponential for nested inversions.

TODO (Daniel): I think we get can something like $\|(N^{-1})_{I,}\|_F=O(\kappa^s)$ and where $s$ is the number of gates (maybe even just depth), and $|N^{-1}\|_F=O(\kappa^{2s})$. I will need to check this.
Can we get a bound in terms of the naive norm bound of the original formula using $\|A+B\|_F\le\|A\|_F+\|B\|_F$ and $\|AB\|_F\le\|A\|_F\|B\|_F$?

\paragraph{One gate}
$M_v$ is the $n_v\times m_v$ input matrix.

\begin{align*}
    N^{-1}=N&=\begin{bmatrix}
        I^{(n_v)}&M_v\\
        0^{(m_v,n_v)}&-I^{(m_v)}
    \end{bmatrix}\\
    \|(N^{-1})_{I,}\|&\le \|M_v\|_F+\sqrt{m_v}\\
    \|N^{-1}\|_F=\|N\|_F&\le \sqrt{n_v+m_v}+\|M_v\|_F
\end{align*}

\paragraph{Inversion}

$N'$ is a $n_{N'}\times n_{N'}$ matrix. $(N'^{-1})_{I',J'}$ is the $n_w\times n_w$ matrix that the child node $w$ outputs.
\begin{align*}
    N&=\begin{bmatrix}
        N'&-I^{(n_{N'})}_{,J'}\\
        I^{(n_{N'})}_{I',}&0^{(n_w,n_w)}
    \end{bmatrix}\\
    N^{-1}&=\begin{bmatrix}
        N'^{-1}-(N'^{-1})_{,J'}(N'^{-1})_{I',J'}^{-1}(N'^{-1})_{I',}& (N'^{-1})_{,J'}(N'^{-1})_{I',J'}^{-1}\\
        -(N'^{-1})_{I',J'}^{-1}(N'^{-1})_{I',}&(N'^{-1})_{I',J'}^{-1}
    \end{bmatrix}\\
    \|N\|_F&\le \|N'\|_F+\sqrt{2n_w}\\
    \|(N^{-1})_{I,}\|_F&\le \|(N'^{-1})_{I',J'}^{-1}\|_F(1+\|(N'^{-1})_{I',}\|_F)\\
    \|N^{-1}\|_F&\le \|N'^{-1}\|_F+\|((N'^{-1})_{I',J'})^{-1}\|_F(\|(N'^{-1})_{I',}\|_F+1)(\|(N'^{-1})_{,J'}\|_F+1)
\end{align*}



\paragraph{Addition and Subtraction}

$L$ is a $n_L\times n_L$ matrix and $R$ is a $n_R\times n_R$ matrix.

The outputs of the children gates are $(L^{-1})_{I_L,J_L}$ and $(R^{-1})_{I_R,J_R}$, which are $n_w\times m_w$ matrices.

This is the same formula for $N$ as in the SOSA paper up except the last two rows are swapped, then the last row and column are negated.
\begin{align*}
    N&=\begin{bmatrix}
        L&0&I^{(n_L)}_{,J_L}&0\\
        0&R&I^{(n_R)}_{,J_R}&0\\
        I^{(n_L)}_{I_L,}&I^{(n_R)}_{I_R,}&0&I^{(n_w)}\\
        0&0&I^{(m_w)}&0
    \end{bmatrix}\\
    N^{-1}&=\begin{bmatrix}
        L^{-1}&0&0&-(L^{-1})_{,J_L}\\
        0&R^{-1}&0&-(R^{-1})_{,J_R}\\
        0&0&0&I^{(m_w)}\\
        -(L^{-1})_{I_L,}&-(R^{-1})_{I_R,}&I^{(n_w)}&(L^{-1})_{I_L,J_L}+(R^{-1})_{I_R,J_R}\\
    \end{bmatrix}\\
    \|N\|_F&\le \|L^{-1}\|_F+\|R^{-1}\|_F+\sqrt{3n_w+3m_w}\\
    \|(N^{-1})_{I,}\|_F&\le \|(L^{-1})_{I_L,}\|_F+\|(R^{-1})_{J_L,}\|_F+\|(L^{-1})_{I_L,J_L}\|_F+\|(R^{-1})_{I_R,J_R}\|_F+\sqrt{n_w}\\
    \|N^{-1}\|_F&\le \|L^{-1}\|_F+\|R^{-1}\|_F+\|(L^{-1})_{I_L,}\|_F+\|(L^{-1})_{,J_L}\|_F+\|(R^{-1})_{I_R,}\|_F+\|(R^{-1})_{,J_R}\|_F+\sqrt{n_w+m_w}
\end{align*}

Subtraction is the same with a few sign changes in the matrices.

\paragraph{Multiplication}
$L$ is a $n_L\times n_L$ matrix, $R$ is a $n_R\times n_R$ matrix.

The outputs of the children gates are $(L^{-1})_{I_L,J_L}$ and $(R^{-1})_{I_R,J_R}$.

\begin{align*}
    N&=\begin{bmatrix}
        L&-I^{(n_L)}_{[n_L],J_L}I^{(n_R)}_{I_R,[n_R]}\\
        0^{(n_R,n_L)}&R
    \end{bmatrix}\\
    N^{-1}&=\begin{bmatrix}
        L^{-1}&(L^{-1})_{,J_L}(R^{-1})_{I_R,}\\
        0&R^{-1}
    \end{bmatrix}\\
    \|N\|_F&\le \|L\|_F+\|R\|_F+\sqrt{n_Ln_R}\\
    \|(N^{-1})_{I,}\|_F&\le \|(L^{-1})_{I_L,}\|_F+\|(L^{-1})_{I_L,J_L}\|_F\|(R^{-1})_{I_R,}\|_F\\
    \|N^{-1}\|_F&\le \|L^{-1}\|_F+\|R^{-1}\|_F+\|(L^{-1})_{,J_L}\|_F\|(R^{-1})_{I_R,}\|_F
\end{align*}

\section{Additional notes}

Remark: the addition gate should generalize straightforwardly to $n$-ary addition.

Remark: we could get a $-(L+R)^{-1}$ gate by taking the bottom-right block of

\begin{align*}
    \begin{bmatrix}
        L&0&I^{(n_L)}_{,J_L}\\
        0&R&I^{(n_R)}_{,J_R}\\
        I^{(n_L)}_{I_L,}&I^{(n_R)}_{I_R,}&0
    \end{bmatrix}^{-1}
\end{align*}

which is shorter.

In fact, the current addition gate (the one in SOSA with last two rows swapped, and last row and column negated) can be viewed as $-(-(L+R)^{-1})^{-1}$ using this, but it somehow avoids problems when $L+R$ is not invertible.

\paragraph{Regarding symmetric gates}

All output matrices will be on the diagonal.

Instead of one gate we can just put in the actual matrix (which gets inverted) and apply the inverse gate. Like the addition gate, the result should not dependd on $M$ actually being invertible.

The addition gate looks more symmetric if we swap the last two rows.

The inversion gate can be made a symmetric $-A^{-1}$ gate by removing the minus sign.

Can we even do scalar multiplication by $-1$? I suppose that could be pushed down into the input gates.

$A\mapsto CAC^\top$ for constant $C$ an be done by taking the negative-inverse-of-sum gate and replacing the row/column selectors with $C$.

\section{Concrete norm bounds}


Suppose the output of any gate has Frobenius norm bounded by $\kappa\ge \max_v(n_v+m_v)$. (Maybe a better assumption will be bounded by $\kappa^s$?)

Observe that $(\kappa+1)^a+(\kappa+1)^b\le (\kappa+1)^{a+b}$ for $a,b\ge 1$, since $((\kappa+1)^a-1)((\kappa+1)^b-1)\ge 1$.


We will show that $f(a)=3\alpha\kappa$ is an upper bound of $\|N\|_F$ where $N$ is the matrix output of a circuit with $a$ gates.

It suffices to show that
\begin{align*}
    f(1)&\ge 2\kappa&  \text{One}\\
    f(a+1)&\ge f(a)+2\kappa&\text{Inverse}\\
    f(a+b+1)&\ge f(a)+f(b)+3\kappa&\text{Addition/subtraction}\\
    f(a+b+1)&\ge f(b)+f(b)+\kappa&\text{Multiplication}
\end{align*}

We will show that $g(a)=3(\kappa+1)^a$ is an upper bound for $\|(N^{-1})_{I,}\|_F$ (and symmetrically, $\|(N^{-1})_{,J}\|_F$)

It suffices to show that
\begin{align*}
    g(1)&\ge 2\kappa\\
    g(a+1)&\ge \kappa+\kappa g(a)\\
    g(a+b+1)&\ge g(a)+g(b)+3\kappa\\
    g(a+b+1)&\ge g(a)+\kappa g(b)
\end{align*}

\begin{align*}
    2\kappa&\le 3(\kappa+1)^1\\
    \kappa+\kappa\cdot 3(\kappa+1)^a
    &\le 3[\kappa+\kappa(\kappa+1)^a]\\
    &\le 3[(\kappa+1)^a+\kappa(\kappa+1)^a]\\
 &=3(\kappa+1)^{a+1}\\
 3(\kappa+1)^a+3(\kappa+1)^b+3\kappa&\le 3(\kappa+1)^{a+b}+3\kappa\\
 &\le 3(\kappa+1)^{a+b}+3\kappa(\kappa+1)^{a+b}\\
 &=3(\kappa+1)^{a+b+1}\\
 3(\kappa+1)^a+\kappa(\kappa+1)^b&\le 3\kappa[(\kappa+1)^a+(\kappa+1)^b]\\
 &\le 3\kappa(\kappa+1)^{a+b}\\
 &\le 3(\kappa+1)^{a+b+1}
\end{align*}


We will show that $h(a)=16(\kappa+1)^{2a+1}$ is an upper bound for $\|N^{-1}\|_F$.

It suffices to show that
\begin{align*}
    h(1)&\ge 3\kappa\\
    h(a+1)&\ge h(a)+\kappa(g(a)+1)^2\\
    h(a+b+1)&\ge h(a)+h(b)+2g(a)+2g(b)+2\kappa\\
    h(a+b+1)&\ge h(a)+h(b)+g(a)g(b)
\end{align*}

\begin{align*}
    3\kappa&\le 16(\kappa+1)^3\\
    16(\kappa+1)^{2a+1}+\kappa(3(\kappa+1)^a+1)^2&\le 16(\kappa+1)^{2a+1}+16(\kappa+1)^{2a+1}\\
    &\le 16(\kappa+1)^{2(a+1)+1}\\
    16(\kappa+1)^{2a+1}+16(\kappa+1)^{2b+1}+2[3(\kappa+1)^a+3(\kappa+1)^b]+2\kappa&\le 
    16(\kappa+1)^{2a+2b+2}+6(\kappa+1)^{a+b}+2\kappa\\
    &\le
    16(\kappa+1)^{2a+2b+2}+16(\kappa+1)^{a+b}\\
    &\le 
    16(\kappa+1)^{2(a+b+1)+1}
\end{align*}

\section{Norm Bounds (Formal Rewrite)}
We use the same notation as \cite{van2021unifying}with the additional abbreviation that $A_{I,}=A_{I,[n]}$ and $A_{,J}=A_{[m],J}$ for $A\in\R^{m\times n}$

\begin{lemma}

    
    Let $f$ be a $p$-input matrix formula over $\R$ using $s$ gates. Suppose $N$, $I$, and $J$ are constructed as in Theorem 3.1 of \cite{van2021unifying} so that $(N^{-1})_{I,J}=f(A_1,\ldots,A_p)$.

    Let $\kappa\ge \max_{v\in V}n_v+m_v$.
    
    Suppose $e,f,g,h:\mathbb{N}\to\mathbb{R}_{\ge 0}$ satisfy for all integer $a,b\ge 1$,
\begin{align*}
    e(1)&\ge \kappa\\
    e(a+1)&\ge \kappa\\
    e(a+b+1)&\ge e(a)+e(b)\\
    e(a+b+1)&\ge e(a)e(b)\\
    f(1)&\ge 2\kappa\\
    f(a+1)&\ge f(a)+2\kappa\\
    f(a+b+1)&\ge f(a)+f(b)+2\kappa\\
    f(a+b+1)&\ge f(b)+f(b)+\kappa\\
    g(1)&\ge 2\kappa\\
    g(a+1)&\ge \kappa+\kappa g(a)\\
    g(a+b+1)&\ge g(a)+g(b)+e(a)+e(b)+\kappa\\
    g(a+b+1)&\ge g(a)+e(a) g(b)\\
    h(1)&\ge 2\kappa\\
    h(a+1)&\ge h(a)+\kappa(g(a)+1)^2\\
    h(a+b+1)&\ge h(a)+h(b)+2g(a)+2g(b)+\kappa\\
    h(a+b+1)&\ge h(a)+h(b)+g(a)g(b)
\end{align*}
    
    {\color{red}Daniel: Should rename one $f$ to something else.}
    
    Then, if $\|A_1\|_F,\ldots,\|A_p\|_F\le \kappa$, and the Frobenius norms of outputs of intermediate inverse gates are also bounded by $\kappa$, we have
    \begin{align*}
        \|N\|_F&\le f(s)\\
        \|N^{-1}\|_F&\le h(s)
    \end{align*}
\end{lemma}
\begin{proof}
    We will show by induction on $s\ge 1$ that
    \begin{align*}
        \|N\|_F&\le f(s) &\|(N^{-1})_{I,J}\|_F&\le e(s) &\|(N^{-1})_{I,}\|_F&\le g(s)&
        \|(N^{-1})_{,J}\|_F&\le g(s)&\|N^{-1}\|_F&\le h(s)
    \end{align*}

    The base case is when $s=1$, in which case the formula consists of a single one gate.

    We have
\begin{align*}
    N^{-1}=N&=\begin{bmatrix}
        I^{(n_v)}&M_v\\
        0^{(m_v,n_v)}&-I^{(m_v)}
    \end{bmatrix}
\end{align*}
where $M_v$ is one of the input matrices, and hence $\|M_v\|_F\le \kappa$. By the triangle inequality,
\begin{align*}
    \|N\|_F&\le \sqrt{n_v+m_v}+\|M_v\|_F\le 2\kappa\le f(1)\\
    \|(N^{-1})_{I,J}\|&\le \|M_v\|_F\le \kappa\le e(1)\\
    \|(N^{-1})_{I,}\|&\le \|M_v\|_F+\sqrt{n_v}\le 2\kappa\le g(1)\\
    \|(N^{-1})_{,J}\|&\le \|M_v\|_F+\sqrt{m_v}\le 2\kappa\le g(1)\\
    \|N^{-1}\|_F&\le \sqrt{n_v+m_v}+\|M_v\|_F\le 2\kappa\le h(1)
\end{align*}

Now we do the inductive step.
\paragraph{Inversion}
Suppose the last gate is a inversion gate. Suppose $N'$ is a $n_{N'}\times n_{N'}$ matrix such that $(N'^{-1})_{I',J'}$ is the $n_w\times n_w$ matrix that the child node $w$ outputs. The child node has $a=s-1\ge 1$ gates.
\begin{align*}
    N&=\begin{bmatrix}
        N'&-I^{(n_{N'})}_{,J'}\\
        I^{(n_{N'})}_{I',}&0^{(n_w,n_w)}
    \end{bmatrix}\\
    N^{-1}&=\begin{bmatrix}
        N'^{-1}-(N'^{-1})_{,J'}(N'^{-1})_{I',J'}^{-1}(N'^{-1})_{I',}& (N'^{-1})_{,J'}(N'^{-1})_{I',J'}^{-1}\\
        -(N'^{-1})_{I',J'}^{-1}(N'^{-1})_{I',}&(N'^{-1})_{I',J'}^{-1}
    \end{bmatrix}\\
    \|N\|_F&\le \|N'\|_F+\sqrt{2n_w}\\
    &\le f(a)+2\kappa\le f(a+1)=f(s)\\
    \|(N^{-1})_{I,J}\|_F&=\|(N'^{-1})_{I',J'}^{-1}\|_F\le \kappa\le e(s)&\text{by assumption}\\
    \|(N^{-1})_{I,}\|_F&\le \|(N'^{-1})_{I',J'}^{-1}\|_F(1+\|(N'^{-1})_{I',}\|_F)\\
    &\le \kappa(1+g(a))\le g(a+1)=g(s)\\
    \|(N^{-1})_{,J}\|_F&\le \|(N'^{-1})_{I',J'}^{-1}\|_F(1+\|(N'^{-1})_{,J'}\|_F)\\
    &\le \kappa(1+g(a))\le g(a+1)=g(s)\\
    \|N^{-1}\|_F&\le \|N'^{-1}\|_F+\|(N'^{-1})_{I',J'}^{-1}\|_F(\|(N'^{-1})_{I',}\|_F+1)(\|(N'^{-1})_{,J'}\|_F+1)\\
    &\le h(a)+\kappa(g(a)+1)^2\le h(a+1)=h(s)
\end{align*}
\paragraph{Addition}
Suppose the last gate was an addition gate.

Suppose the left child has $a\ge 1$ gates and the right child has $b\ge 1$ gates, where $s=a+b+1$.

Let $L$ be the $n_L\times n_L$ matrix and $R$ be the a $n_R\times n_R$ matrix such that the outputs of the child gates are $(L^{-1})_{I_L,J_L}$ and $(R^{-1})_{I_R,J_R}$, which are $n_w\times m_w$ matrices.

This is the same formula for $N$ as in the SOSA paper up except the last two rows are swapped, then the last row and column are negated. {\color{red} Daniel: Should I use the original formula for consistency? The norms are unaffected.}
{\color{red}Daniel: also, the superscripts on $0$s are missing. I fell like this is clearer?}\jan{yes, removing superscripts on 0 is fine.}
\begin{align*}
    N&=\begin{bmatrix}
        L&0&I^{(n_L)}_{,J_L}&0\\
        0&R&I^{(n_R)}_{,J_R}&0\\
        I^{(n_L)}_{I_L,}&I^{(n_R)}_{I_R,}&0&I^{(n_w)}\\
        0&0&I^{(m_w)}&0
    \end{bmatrix}\\
    N^{-1}&=\begin{bmatrix}
        L^{-1}&0&0&-(L^{-1})_{,J_L}\\
        0&R^{-1}&0&-(R^{-1})_{,J_R}\\
        0&0&0&I^{(m_w)}\\
        -(L^{-1})_{I_L,}&-(R^{-1})_{I_R,}&I^{(n_w)}&(L^{-1})_{I_L,J_L}+(R^{-1})_{I_R,J_R}\\
    \end{bmatrix}\\
    \|N\|_F&\le \|L\|_F+\|R\|_F+\sqrt{3n_w+3m_w}\\
    &\le f(a)+f(b)+2\kappa\le f(a+b+1)=f(s)\\
    \|(N^{-1})_{I,J}\|_F&\le \|(L^{-1})_{I_L,J_L}\|_F+\|(R^{-1})_{I_R,J_R}\|_F\\
    &\le e(a)+e(b)\le e(a+b+1)=e(s)\\
    \|(N^{-1})_{I,}\|_F&\le \|(L^{-1})_{I_L,}\|_F+\|(R^{-1})_{I_R,}\|_F+\|(L^{-1})_{I_L,J_L}\|_F+\|(R^{-1})_{I_R,J_R}\|_F+\sqrt{n_w}\\
    &\le g(a)+g(b)+e(a)+e(b)+\kappa\le g(a+b+1)=g(s)\\
    \|(N^{-1})_{,J}\|_F&\le \|(L^{-1})_{,J_L}\|_F+\|(R^{-1})_{,J_R}\|_F+\|(L^{-1})_{I_L,J_L}\|_F+\|(R^{-1})_{I_R,J_R}\|_F+\sqrt{m_w}\\
    &\le g(a)+g(b)+e(a)+e(b)+\kappa\le g(a+b+1)=g(s)\\
    \|N^{-1}\|_F&\le \|L^{-1}\|_F+\|R^{-1}\|_F+\|(L^{-1})_{I_L,}\|_F+\|(L^{-1})_{,J_L}\|_F+\|(R^{-1})_{I_R,}\|_F+\|(R^{-1})_{,J_R}\|_F+\sqrt{n_w+m_w}\\
    &\le h(a)+h(b)+2g(a)+2g(b)+\kappa\le h(a+b+1)=h(s)
\end{align*}

Subtraction is the same with a few sign changes in the matrices.

\paragraph{Multiplication}
Suppose the last gate was a multiplication gate.

Suppose the left child has $a\ge 1$ gates and the right child has $b\ge 1$ gates, where $s=a+b+1$.

Let $L$ be the $n_L\times n_L$ matrix and $R$ be the $n_R\times n_R$ matrix such that the outputs of the child gates are $(L^{-1})_{I_L,J_L}$ and $(R^{-1})_{I_R,J_R}$.

\begin{align*}
    N&=\begin{bmatrix}
        L&-I^{(n_L)}_{[n_L],J_L}I^{(n_R)}_{I_R,[n_R]}\\
        0^{(n_R,n_L)}&R
    \end{bmatrix}\\
    N^{-1}&=\begin{bmatrix}
        L^{-1}&(L^{-1})_{,J_L}(R^{-1})_{I_R,}\\
        0&R^{-1}
    \end{bmatrix}\\
    \|N\|_F&\le \|L\|_F+\|R\|_F+\sqrt{\min(n_L,n_R)}\\
    &\le f(a)+f(b)+\kappa\le f(a+b+1)=f(s)\\
    \|(N^{-1})_{I,J}\|_F&\le \|(L^{-1})_{I_L,J_L}\|_F\|(R^{-1})_{I_R,J_R}\|_F\\
    &\le e(a)e(b)\le e(a+b+1)=e(s)\\
    \|(N^{-1})_{I,}\|_F&\le \|(L^{-1})_{I_L,}\|_F+\|(L^{-1})_{I_L,J_L}\|_F\|(R^{-1})_{I_R,}\|_F\\
    &\le g(a)+e(a)g(b)\le g(a+b+1)=g(s)\\
    \|(N^{-1})_{,J}\|_F&\le \|(R^{-1})_{,J_R}\|_F+\|(R^{-1})_{I_R,J_R}\|_F\|(L^{-1})_{,J_L}\|_F\\
    &\le g(b)+e(b)g(a)\le g(a+b+1)=g(s)\\
    \|N^{-1}\|_F&\le \|L^{-1}\|_F+\|R^{-1}\|_F+\|(L^{-1})_{,J_L}\|_F\|(R^{-1})_{I_R,}\|_F\\
    &\le h(a)+h(b)+g(a)g(b)\le h(a+b+1)=h(s)
\end{align*}

\end{proof}

\begin{lemma}
    The functions
    \begin{align*}
        e(a)&=\kappa^a\\
        f(a)&=2a\kappa\\
        g(a)&=(5\kappa)^a\\
        h(a)&=(10\kappa)^{2a+1}
    \end{align*}
    satisfy the hypothesis of {\color{red} cite previous lemma}.

    In particular, we have $\|N\|_F\le 2a\kappa$ and $\|N^{-1}\|_F\le (10\kappa)^{2a+1}$ in the previous lemma.

    {\color{red} Daniel: I can reduce the coefficients $5$ and $10$ if necessary, but the $\kappa^{2a+1}$ seems to be necessary.}
\end{lemma}

\begin{proof}
{\color{red} Daniel: Do we need all of this? Some of these calculations are pretty obvious...}

For $e(a)=\kappa^a$:
\begin{align*}
    \kappa&\le \kappa^1=e(1)\\
    \kappa&\le \kappa^{a+1}=e(a+1)\\
    e(a)+e(b)&=\kappa^a+\kappa^b\le 2\kappa^{a+b}\le \kappa^{a+b+1}=e(a+b+1)\\
    e(a)e(b)&=\kappa^a\kappa^b\le \kappa^{a+b+1}=e(a+b+1)
\end{align*}

{\color{red} Daniel: This used $\kappa\ge n_v+m_v\ge 2$}.

Fo $f(a)=2a\kappa$:
\begin{align*}
    2\kappa&\le 2\cdot 1\kappa=f(1)\\
    f(a)+2\kappa&\le 2a\kappa+2\kappa=f(a+1)\\
    f(a)+f(b)+2\kappa&\le 2a\kappa+2b\kappa+2\kappa=f(a+b+1)\\
    f(a)+f(b)+2\kappa&\le 2a\kappa+2b\kappa+2\kappa\le f(a+b+1)
\end{align*}

For $g(a)=(5\kappa)^a$:
\begin{align*}
    2\kappa&\le 5\kappa=g(1)\\
    \kappa+\kappa g(a)&=\kappa+\kappa(5\kappa)\le (5\kappa)^{a+1}=g(a+1)\\
    g(a)+g(b)+e(a)+e(b)+\kappa&=(5\kappa)^a+(5\kappa)^b+\kappa^a+\kappa^b+\kappa\le 5(5\kappa)^{a+b}\le (5\kappa)^{a+b+1}=g(a+b+1)\\
    g(a)+e(a)g(b)&=(5\kappa)^a+\kappa^a(5\kappa)^b\le (5\kappa)^{a+b}+(5\kappa)^{a+b}\le (5\kappa)^{a+b+1}=g(a+b+1)
\end{align*}

For $h(a)=(10\kappa)^{2a+1}$:
\begin{align*}
    2\kappa&\le (10\kappa)^3=h(1)\\
    h(a)+\kappa(g(a)+1)^2&=(10\kappa)^{2a+1}+\kappa((5\kappa)^a+1)^2\le (10\kappa)^{2a+1}+\kappa(10\kappa)^{2a}\le (10\kappa)^{2a+3}=h(a+1)\\
    h(a)+h(b)+2g(a)+2g(b)+\kappa&=(10\kappa)^{2a+1}+(10\kappa)^{2b+1}+2(5\kappa)^a+2(5\kappa)^b+\kappa\le 7(10\kappa)^{2a+2b+1}\le (10\kappa)^{2b+2b+3}=h(a+b+1)\\
    h(a)+h(b)+g(a)g(b)&=(10\kappa)^{2a+1}+(10\kappa)^{2b+1}+(5\kappa)^a(5\kappa)^b\le 3(10\kappa)^{2a+2b+1}\le (10\kappa)^{2a+2b+3}=h(a+b+1)
\end{align*}
\end{proof}


\section{Meeting 7/5 Notes}

We can prove by induction that $\det(N)$ is just the product of the determinants of all the matrices that are inverted in the formula (up to sign).
